Mind the Gap when Conditioning Amortised Inference in Sequential Latent-Variable Models

Amortised inference enables scalable learning of sequential latent-variable models (LVMs) with the evidence lower bound (ELBO). In this setting, variational posteriors are often only partially conditioned. While the true posteriors depend, e.g., on the entire sequence of observations, approximate posteriors are only informed by past observations. This mimics the Bayesian filter -- a mixture of smoothing posteriors. Yet, we show that the ELBO objective forces partially-conditioned amortised posteriors to approximate products of smoothing posteriors instead. Consequently, the learned generative model is compromised. We demonstrate these theoretical findings in three scenarios: traffic flow, handwritten digits, and aerial vehicle dynamics. Using fully-conditioned approximate posteriors, performance improves in terms of generative modelling and multi-step prediction.

==> tables/blackbird/blackbird-params-hyperpars-full.tex <==
\begin{tabular}{lll}
\toprule
                                              field &                                              value \\
\midrule
                                       batch\_size &                                                 32 \\
                   optimizer.learning\_rate &                                              0.003 \\
                           optimizer.beta1 &                                                0.8 \\
                                   n\_latent &                                                 20 \\
                            initial.n\_flows &                                                 12 \\
                      initial.layer\_sizes.0 &                                                 16 \\
                      initial.layer\_sizes.1 &                                                  8 \\
                            transition.kind &                                         stochastic \\
                       transition.func\_kind &                                            highway \\
           transition.layers.0.units &                                                 64 \\
      transition.layers.0.activation &                                           softplus \\
           transition.layers.1.units &                                                 16 \\
      transition.layers.1.activation &                                           softplus \\
          inv\_initial.layers.0.units &                                                 32 \\
     inv\_initial.layers.0.activation &                                               tanh \\
          inv\_initial.layers.1.units &                                                128 \\
     inv\_initial.layers.1.activation &                                               relu \\
      inv\_disturbance.layers.0.units &                                                128 \\
 inv\_disturbance.layers.0.activation &                                               tanh \\
      inv\_disturbance.layers.1.units &                                                128 \\
 inv\_disturbance.layers.1.activation &                                               relu \\
                       feature\_rnn.n\_states &                                                128 \\
                       feature\_rnn.n\_layers &                                                  1 \\
                  feature\_rnn.bidirectional &                                               True \\
                      feature\_rnn.cell\_type &                                                gru \\
      feature\_rnn.initial\_mlp.prefix\_length &                                                  7 \\
feature\_rnn.initial\_mlp.layers.0.units&                                                128 \\
feature\_rnn.initial\_mlp.layers.0.activation&                                           softsign \\
feature\_rnn.initial\_mlp.layers.1.units&                                                 32 \\
feature\_rnn.initial\_mlp.layers.1.activation&                                           softplus \\
                        emission.scale\_kind &                                              fixed \\
                             emission.scale &                       array([0.15 , 0.15 , 0.075]) \\
\bottomrule
\end{tabular}



==> tables/blackbird/blackbird-params-hyperpars-semi.tex <==
\begin{tabular}{ll}
\toprule
                                              field &                                              value \\
\midrule
                                      batch\_size &                                                 16 \\
                  optimizer.learning\_rate &                                              0.001 \\
                          optimizer.beta1 &                                                0.9 \\
                                  n\_latent &                                                 22 \\
                           initial.n\_flows &                                                 12 \\
                     initial.layer\_sizes.0 &                                                  8 \\
                     initial.layer\_sizes.1 &                                                  8 \\
                           transition.kind &                                         stochastic \\
                      transition.func\_kind &                                           residual \\
          transition.layers.0.units &                                                 16 \\
     transition.layers.0.activation &                                               tanh \\
          transition.layers.1.units &                                                 32 \\
     transition.layers.1.activation &                                           softplus \\
         inv\_initial.layers.0.units &                                                 16 \\
    inv\_initial.layers.0.activation &                                               tanh \\
         inv\_initial.layers.1.units &                                                 16 \\
    inv\_initial.layers.1.activation &                                           softsign \\
     inv\_disturbance.layers.0.units &                                                 64 \\
inv\_disturbance.layers.0.activation &                                               tanh \\
     inv\_disturbance.layers.1.units &                                                128 \\
inv\_disturbance.layers.1.activation &                                               relu \\
                      feature\_rnn.n\_states &                                                128 \\
                      feature\_rnn.n\_layers &                                                  1 \\
                 feature\_rnn.bidirectional &                                               True \\
                     feature\_rnn.cell\_type &                                                gru \\
     feature\_rnn.initial\_mlp.prefix\_length &                                                  7 \\
eature\_rnn.initial\_mlp.layers.0.units&                                                      32 \\
eature\_rnn.initial\_mlp.layers.0.activation&                                           softplus \\
eature\_rnn.initial\_mlp.layers.1.units&                                                      32 \\
eature\_rnn.initial\_mlp.layers.1.activation&                                           softsign \\
                       emission.scale\_kind &                                              fixed \\
                            emission.scale &                       array([0.15 , 0.15 , 0.075]) \\
\bottomrule
\end{tabular}



==> tables/blackbird/blackbird-template-hyperpars-full.tex <==
\begin{tabular}{lll}
\toprule
                                              field &                                              range \\
\midrule
                                       batch\_size &                       Choice([8, 16, 32, 64, 128]) \\
                   optimizer.learning\_rate &      Choice([0.003, 0.001, 0.0003, 0.0001, 3e-05]) \\
                           optimizer.beta1 &                            Choice([0.5, 0.8, 0.9]) \\
                                   n\_latent &                             Range(low=16, high=33) \\
                            initial.n\_flows &                              Choice([2, 4, 8, 12]) \\
                      initial.layer\_sizes.0 &                            Choice([8, 16, 32, 64]) \\
                      initial.layer\_sizes.1 &                            Choice([8, 16, 32, 64]) \\
                            transition.kind &                                         stochastic \\
                       transition.func\_kind &           Choice(['residual', 'highway', 'plain']) \\
           transition.layers.0.units &                     Choice([16, 32, 64, 128, 192]) \\
      transition.layers.0.activation &   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
           transition.layers.1.units &                     Choice([16, 32, 64, 128, 192]) \\
      transition.layers.1.activation &   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
          inv\_initial.layers.0.units &                          Choice([16, 32, 64, 128]) \\
     inv\_initial.layers.0.activation &   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
          inv\_initial.layers.1.units &                          Choice([16, 32, 64, 128]) \\
     inv\_initial.layers.1.activation &   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
      inv\_disturbance.layers.0.units &                          Choice([16, 32, 64, 128]) \\
 inv\_disturbance.layers.0.activation &   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
      inv\_disturbance.layers.1.units &                          Choice([16, 32, 64, 128]) \\
 inv\_disturbance.layers.1.activation &   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
                       feature\_rnn.n\_states &                              Choice([32, 64, 128]) \\
                       feature\_rnn.n\_layers &                                     Choice([1, 2]) \\
                  feature\_rnn.bidirectional &                                               True \\
                      feature\_rnn.cell\_type &                                                gru \\
      feature\_rnn.initial\_mlp.prefix\_length &                                                  7 \\
feature\_rnn.initial\_mlp.layers.0.units&                               Choice([16, 32, 64, 128]) \\
feature\_rnn.initial\_mlp.layers.0.activation&   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
feature\_rnn.initial\_mlp.layers.1.units&                               Choice([16, 32, 64, 128]) \\
feature\_rnn.initial\_mlp.layers.1.activation&   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
                        emission.scale\_kind &                                              fixed \\
                             emission.scale &                       array([0.15 , 0.15 , 0.075]) \\
\bottomrule
\end{tabular}



==> tables/blackbird/blackbird-template-hyperpars-semi.tex <==
\begin{tabular}{ll}
\toprule
                                              field &                                              range \\
\midrule
                                        batch\_size &                       Choice([8, 16, 32, 64, 128]) \\
                    optimizer.learning\_rate &      Choice([0.003, 0.001, 0.0003, 0.0001, 3e-05]) \\
                            optimizer.beta1 &                            Choice([0.5, 0.8, 0.9]) \\
                                    n\_latent &                             Range(low=16, high=33) \\
                             initial.n\_flows &                              Choice([2, 4, 8, 12]) \\
                       initial.layer\_sizes.0 &                            Choice([8, 16, 32, 64]) \\
                       initial.layer\_sizes.1 &                            Choice([8, 16, 32, 64]) \\
                             transition.kind &                                         stochastic \\
                        transition.func\_kind &           Choice(['residual', 'highway', 'plain']) \\
            transition.layers.0.units &                     Choice([16, 32, 64, 128, 192]) \\
       transition.layers.0.activation &   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
            transition.layers.1.units &                     Choice([16, 32, 64, 128, 192]) \\
       transition.layers.1.activation &   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
           inv\_initial.layers.0.units &                          Choice([16, 32, 64, 128]) \\
      inv\_initial.layers.0.activation &   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
           inv\_initial.layers.1.units &                          Choice([16, 32, 64, 128]) \\
      inv\_initial.layers.1.activation &   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
       inv\_disturbance.layers.0.units &                          Choice([16, 32, 64, 128]) \\
  inv\_disturbance.layers.0.activation &   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
       inv\_disturbance.layers.1.units &                          Choice([16, 32, 64, 128]) \\
  inv\_disturbance.layers.1.activation &   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
                        feature\_rnn.n\_states &                              Choice([32, 64, 128]) \\
                        feature\_rnn.n\_layers &                                     Choice([1, 2]) \\
                   feature\_rnn.bidirectional &                                               True \\
                       feature\_rnn.cell\_type &                                                gru \\
       feature\_rnn.initial\_mlp.prefix\_length &                                                  7 \\
 feature\_rnn.initial\_mlp.layers.0.... &                          Choice([16, 32, 64, 128]) \\
 feature\_rnn.initial\_mlp.layers.0.... &   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
 feature\_rnn.initial\_mlp.layers.1.... &                          Choice([16, 32, 64, 128]) \\
 feature\_rnn.initial\_mlp.layers.1.... &   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
                         emission.scale\_kind &                                              fixed \\
                              emission.scale &                       array([0.15 , 0.15 , 0.075]) \\
\bottomrule
\end{tabular}



==> tables/rowing-mnist/rowing-mnist-hyperpars-under.tex <==
\begin{tabular}{lll}
\toprule
                                              field &                                              range \\
\midrule
                                         batch\_size &                                                 32 \\
                     optimizer.learning\_rate &                                              0.003 \\
                             optimizer.beta1 &                                                0.8 \\
                                     n\_latent &                                                 25 \\
                              initial.n\_flows &                                                 12 \\
                        initial.layer\_sizes.0 &                                                 64 \\
                        initial.layer\_sizes.1 &                                                 32 \\
                          emission.scale\_kind &                                          learnable \\
                               emission.scale &                                                0.2 \\
               emission.layers.0.units &                                                 16 \\
          emission.layers.0.activation &                                               relu \\
               emission.layers.1.units &                                                 32 \\
          emission.layers.1.activation &                                           softplus \\
                              transition.kind &                                         stochastic \\
                         transition.func\_kind &                                            highway \\
             transition.layers.0.units &                                                 32 \\
        transition.layers.0.activation &                                           softsign \\
             transition.layers.1.units &                                                128 \\
        transition.layers.1.activation &                                           softplus \\
            inv\_initial.layers.0.units &                                                 32 \\
       inv\_initial.layers.0.activation &                                           softsign \\
            inv\_initial.layers.1.units &                                                 64 \\
       inv\_initial.layers.1.activation &                                               tanh \\
        inv\_disturbance.layers.0.units &                                                 64 \\
   inv\_disturbance.layers.0.activation &                                           softplus \\
        inv\_disturbance.layers.1.units &                                                 64 \\
   inv\_disturbance.layers.1.activation &                                           softsign \\
                         feature\_rnn.n\_states &                                                128 \\
                    feature\_rnn.bidirectional &                                               True \\
                        feature\_rnn.cell\_type &                                                gru \\
        feature\_rnn.initial\_mlp.prefix\_length &                                                  1 \\
  feature\_rnn.initial\_mlp.layers.0.units &                                                 16 \\
  feature\_rnn.initial\_mlp.layers.1.units &                                                 32 \\
  feature\_rnn.initial\_mlp.layers.0.activation &                                           softplus \\
  feature\_rnn.initial\_mlp.layers.1.activation &                                           softsign \\
\bottomrule
\end{tabular}



==> tables/rowing-mnist/rowing-mnist-params-hyperpars-full.tex <==
\begin{tabular}{lll}
\toprule
                                              field &                                              value \\
\midrule
                                         batch\_size &                                                128 \\
                     optimizer.learning\_rate &                                              0.003 \\
                             optimizer.beta1 &                                                0.9 \\
                                     n\_latent &                                                 25 \\
                              initial.n\_flows &                                                  4 \\
                        initial.layer\_sizes.0 &                                                 64 \\
                        initial.layer\_sizes.1 &                                                 32 \\
                          emission.scale\_kind &                                          learnable \\
                               emission.scale &                                               0.02 \\
               emission.layers.0.units &                                                 64 \\
          emission.layers.0.activation &                                           softsign \\
               emission.layers.1.units &                                                 64 \\
          emission.layers.1.activation &                                           softplus \\
                              transition.kind &                                         stochastic \\
                         transition.func\_kind &                                            highway \\
             transition.layers.0.units &                                                192 \\
        transition.layers.0.activation &                                               relu \\
             transition.layers.1.units &                                                192 \\
        transition.layers.1.activation &                                               tanh \\
            inv\_initial.layers.0.units &                                                 64 \\
       inv\_initial.layers.0.activation &                                           softsign \\
            inv\_initial.layers.1.units &                                                 16 \\
       inv\_initial.layers.1.activation &                                               relu \\
        inv\_disturbance.layers.0.units &                                                 64 \\
   inv\_disturbance.layers.0.activation &                                               relu \\
        inv\_disturbance.layers.1.units &                                                 16 \\
   inv\_disturbance.layers.1.activation &                                           softsign \\
                         feature\_rnn.n\_states &                                                 32 \\
                    feature\_rnn.bidirectional &                                               True \\
                        feature\_rnn.cell\_type &                                                gru \\
        feature\_rnn.initial\_mlp.prefix\_length &                                                  1 \\
  feature\_rnn.initial\_mlp.layers.0.units &                                                 16 \\
  feature\_rnn.initial\_mlp.layers.0.activation &                                               tanh \\
  feature\_rnn.initial\_mlp.layers.1.units&                                                128 \\
  feature\_rnn.initial\_mlp.layers.1.activation &                                           softplus \\
\bottomrule
\end{tabular}



==> tables/traffic-flow/traffic-flow-params-hyperpars-full.tex <==
\begin{tabular}{lll}
\toprule
                                              field &                                              value \\
\midrule
                                       batch\_size &                                                  8 \\
                   optimizer.learning\_rate &                                             0.0003 \\
                           optimizer.beta1 &                                                0.8 \\
                                   n\_latent &                                                 64 \\
                            initial.n\_flows &                                                  4 \\
                      initial.layer\_sizes.0 &                                                  8 \\
                      initial.layer\_sizes.1 &                                                  8 \\
                            transition.kind &                                         stochastic \\
                       transition.func\_kind &                                              plain \\
           transition.layers.0.units &                                                 64 \\
      transition.layers.0.activation &                                           softsign \\
transition.layers.0.kernel\_initia... &                                         orthogonal \\
          inv\_initial.layers.0.units &                                                 64 \\
     inv\_initial.layers.0.activation &                                           softplus \\
inv\_initial.layers.0.kernel\_initi... &                                      glorot\_normal \\
      inv\_disturbance.layers.0.units &                                                 64 \\
 inv\_disturbance.layers.0.activation &                                           softplus \\
inv\_disturbance.layers.0.kernel\_i... &                                      glorot\_normal \\
                       feature\_rnn.n\_states &                                                 64 \\
                       feature\_rnn.n\_layers &                                                  1 \\
                  feature\_rnn.bidirectional &                                               True \\
                      feature\_rnn.cell\_type &                                                gru \\
      feature\_rnn.initial\_mlp.prefix\_length &                                                  7 \\
feature\_rnn.initial\_mlp.layers.0.units &                                                 64 \\
feature\_rnn.initial\_mlp.layers.0.activation &                                               relu \\
feature\_rnn.initial\_mlp.layers.1.units &                                                 32 \\
feature\_rnn.initial\_mlp.layers.1.activation &                                           softsign \\
                        emission.scale\_kind &                                              fixed \\
                             emission.scale &                                            1.28276 \\
             emission.layers.0.units &                                                 64 \\
        emission.layers.0.activation &                                           softplus \\
emission.layers.0.kernel\_initializer &                                      glorot\_normal \\
                                   n\_hidden &                                                 64 \\
\bottomrule
\end{tabular}


==> tables/traffic-flow/traffic-flow-params-hyperpars-semi.tex <==
\begin{tabular}{lll}
\toprule
                                             field &                                              value \\
\midrule
                                       batch\_size &                                                128 \\
                   optimizer.learning\_rate &                                             0.0003 \\
                           optimizer.beta1 &                                                0.5 \\
                                   n\_latent &                                                 64 \\
                            initial.n\_flows &                                                  4 \\
                      initial.layer\_sizes.0 &                                                  8 \\
                      initial.layer\_sizes.1 &                                                 32 \\
                            transition.kind &                                         stochastic \\
                       transition.func\_kind &                                              plain \\
           transition.layers.0.units &                                                 64 \\
      transition.layers.0.activation &                                           softsign \\
transition.layers.0.kernel\_initia... &                                         orthogonal \\
          inv\_initial.layers.0.units &                                                 64 \\
     inv\_initial.layers.0.activation &                                           softplus \\
inv\_initial.layers.0.kernel\_initi... &                                      glorot\_normal \\
      inv\_disturbance.layers.0.units &                                                 64 \\
 inv\_disturbance.layers.0.activation &                                           softplus \\
inv\_disturbance.layers.0.kernel\_i... &                                      glorot\_normal \\
                       feature\_rnn.n\_states &                                                 64 \\
                       feature\_rnn.n\_layers &                                                  1 \\
                  feature\_rnn.bidirectional &                                               True \\
                      feature\_rnn.cell\_type &                                                gru \\
      feature\_rnn.initial\_mlp.prefix\_length &                                                  7 \\
feature\_rnn.initial\_mlp.layers.0.units &                                                128 \\
feature\_rnn.initial\_mlp.layers.1.units &                                                 16 \\
feature\_rnn.initial\_mlp.layers.0.activation &                                           softsign \\
feature\_rnn.initial\_mlp.layers.1.activation &                                               tanh \\
                        emission.scale\_kind &                                              fixed \\
                             emission.scale &                                           0.775862 \\
             emission.layers.0.units &                                                 64 \\
        emission.layers.0.activation &                                           softplus \\
emission.layers.0.kernel\_initializer &                                      glorot\_normal \\
                                   n\_hidden &                                                 64 \\
\bottomrule
\end{tabular}



==> tables/traffic-flow/traffic-flow-params-hyperpars-under.tex <==
\begin{tabular}{lll}
\toprule
                                             field &                                              value \\
\midrule
                                        batch\_size &                                                  8 \\
                    optimizer.learning\_rate &                                             0.0001 \\
                            optimizer.beta1 &                                                0.5 \\
                                    n\_latent &                                                 64 \\
                             initial.n\_flows &                                                  4 \\
                       initial.layer\_sizes.0 &                                                 32 \\
                       initial.layer\_sizes.1 &                                                 64 \\
                             transition.kind &                                         stochastic \\
                        transition.func\_kind &                                              plain \\
            transition.layers.0.units &                                                 64 \\
       transition.layers.0.activation &                                           softsign \\
 transition.layers.0.kernel\_initia... &                                         orthogonal \\
           inv\_initial.layers.0.units &                                                 64 \\
      inv\_initial.layers.0.activation &                                           softplus \\
 inv\_initial.layers.0.kernel\_initi... &                                      glorot\_normal \\
       inv\_disturbance.layers.0.units &                                                 64 \\
  inv\_disturbance.layers.0.activation &                                           softplus \\
 inv\_disturbance.layers.0.kernel\_i... &                                      glorot\_normal \\
                        feature\_rnn.n\_states &                                                 64 \\
                        feature\_rnn.n\_layers &                                                  1 \\
                   feature\_rnn.bidirectional &                                               True \\
                       feature\_rnn.cell\_type &                                                gru \\
       feature\_rnn.initial\_mlp.prefix\_length &                                                  1 \\
 feature\_rnn.initial\_mlp.layers.0.activation &                                           softsign \\
 feature\_rnn.initial\_mlp.layers.0.units &                                                128 \\
 feature\_rnn.initial\_mlp.layers.1.activation &                                               relu \\
 feature\_rnn.initial\_mlp.layers.1.units &                                                128 \\
                         emission.scale\_kind &                                              fixed \\
                              emission.scale &                                            2.97241 \\
              emission.layers.0.units &                                                 64 \\
         emission.layers.0.activation &                                           softplus \\
 emission.layers.0.kernel\_initializer &                                      glorot\_normal \\
                                    n\_hidden &                                                 64 \\
\bottomrule
\end{tabular}



==> tables/traffic-flow/traffic-flow-template-hyperpars-full.tex <==
\begin{tabular}{lll}
\toprule
                                              field &                                              range \\
\midrule
                                       batch\_size &                       Choice([8, 16, 32, 64, 128]) \\
                   optimizer.learning\_rate &                    Choice([0.0003, 0.0001, 3e-05]) \\
                           optimizer.beta1 &                            Choice([0.5, 0.8, 0.9]) \\
                                   n\_latent &                                                 64 \\
                            initial.n\_flows &                                                  4 \\
                      initial.layer\_sizes.0 &                            Choice([8, 16, 32, 64]) \\
                      initial.layer\_sizes.1 &                            Choice([8, 16, 32, 64]) \\
                            transition.kind &                                         stochastic \\
                       transition.func\_kind &           Choice(['residual', 'highway', 'plain']) \\
           transition.layers.0.units &                                                 64 \\
      transition.layers.0.activation &                                           softsign \\
transition.layers.0.kernel\_initia... &                                         orthogonal \\
          inv\_initial.layers.0.units &                                                 64 \\
     inv\_initial.layers.0.activation &                                           softplus \\
inv\_initial.layers.0.kernel\_initi... &                                      glorot\_normal \\
      inv\_disturbance.layers.0.units &                                                 64 \\
 inv\_disturbance.layers.0.activation &                                           softplus \\
inv\_disturbance.layers.0.kernel\_i... &                                      glorot\_normal \\
                       feature\_rnn.n\_states &                                                 64 \\
                       feature\_rnn.n\_layers &                                                  1 \\
                  feature\_rnn.bidirectional &                                               True \\
                      feature\_rnn.cell\_type &                                                gru \\
      feature\_rnn.initial\_mlp.prefix\_length &                                                  7 \\
feature\_rnn.initial\_mlp.layers.0.units &                          Choice([16, 32, 64, 128]) \\
feature\_rnn.initial\_mlp.layers.0.activation &   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
feature\_rnn.initial\_mlp.layers.1.units &                          Choice([16, 32, 64, 128]) \\
feature\_rnn.initial\_mlp.layers.1.activation &   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
                        emission.scale\_kind &                                              fixed \\
                             emission.scale &  Choice([0.1, 0.2689655172413793, 0.43793103448... \\
             emission.layers.0.units &                                                 64 \\
        emission.layers.0.activation &                                           softplus \\
emission.layers.0.kernel\_initializer &                                      glorot\_normal \\
                                   n\_hidden &                                                 64 \\
\bottomrule
\end{tabular}



==> tables/traffic-flow/traffic-flow-template-hyperpars-semi.tex <==
\begin{tabular}{ll}
\toprule
                                              field &                                              range \\
\midrule
                                        batch\_size &                       Choice([8, 16, 32, 64, 128]) \\
                    optimizer.learning\_rate &                    Choice([0.0003, 0.0001, 3e-05]) \\
                            optimizer.beta1 &                            Choice([0.5, 0.8, 0.9]) \\
                                    n\_latent &                                                 64 \\
                         n\_stationary\_latent &                                                  0 \\
                             initial.n\_flows &                                                  4 \\
                       initial.layer\_sizes.0 &                            Choice([8, 16, 32, 64]) \\
                       initial.layer\_sizes.1 &                            Choice([8, 16, 32, 64]) \\
                             transition.kind &                                         stochastic \\
                        transition.func\_kind &           Choice(['residual', 'highway', 'plain']) \\
            transition.layers.0.units &                                                 64 \\
       transition.layers.0.activation &                                           softsign \\
 transition.layers.0.kernel\_initia... &                                         orthogonal \\
           inv\_initial.layers.0.units &                                                 64 \\
      inv\_initial.layers.0.activation &                                           softplus \\
 inv\_initial.layers.0.kernel\_initi... &                                      glorot\_normal \\
       inv\_disturbance.layers.0.units &                                                 64 \\
  inv\_disturbance.layers.0.activation &                                           softplus \\
 inv\_disturbance.layers.0.kernel\_i... &                                      glorot\_normal \\
                        feature\_rnn.n\_states &                                                 64 \\
                        feature\_rnn.n\_layers &                                                  1 \\
                   feature\_rnn.bidirectional &                                               True \\
                       feature\_rnn.cell\_type &                                                gru \\
       feature\_rnn.initial\_mlp.prefix\_length &                                                  7 \\
 feature\_rnn.initial\_mlp.layers.0.... &                          Choice([16, 32, 64, 128]) \\
 feature\_rnn.initial\_mlp.layers.0.... &   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
 feature\_rnn.initial\_mlp.layers.1.... &                          Choice([16, 32, 64, 128]) \\
 feature\_rnn.initial\_mlp.layers.1.... &   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
                         emission.scale\_kind &                                              fixed \\
                              emission.scale &  Choice([0.1, 0.2689655172413793, 0.43793103448... \\
              emission.layers.0.units &                                                 64 \\
         emission.layers.0.activation &                                           softplus \\
 emission.layers.0.kernel\_initializer &                                      glorot\_normal \\
                                    n\_hidden &                                                 64 \\
\bottomrule
\end{tabular}



==> tables/traffic-flow/traffic-flow-template-hyperpars-under.tex <==
\begin{tabular}{ll}
\toprule
                                              field &                                              range \\
\midrule
                                         batch\_size &                       Choice([8, 16, 32, 64, 128]) \\
                     optimizer.learning\_rate &                    Choice([0.0003, 0.0001, 3e-05]) \\
                             optimizer.beta1 &                            Choice([0.5, 0.8, 0.9]) \\
                                     n\_latent &                                                 64 \\
                          n\_stationary\_latent &                                                  0 \\
                              initial.n\_flows &                                                  4 \\
                        initial.layer\_sizes.0 &                            Choice([8, 16, 32, 64]) \\
                        initial.layer\_sizes.1 &                            Choice([8, 16, 32, 64]) \\
                              transition.kind &                                         stochastic \\
                         transition.func\_kind &           Choice(['residual', 'highway', 'plain']) \\
             transition.layers.0.units &                                                 64 \\
        transition.layers.0.activation &                                           softsign \\
  transition.layers.0.kernel\_initia... &                                         orthogonal \\
            inv\_initial.layers.0.units &                                                 64 \\
       inv\_initial.layers.0.activation &                                           softplus \\
  inv\_initial.layers.0.kernel\_initi... &                                      glorot\_normal \\
        inv\_disturbance.layers.0.units &                                                 64 \\
   inv\_disturbance.layers.0.activation &                                           softplus \\
  inv\_disturbance.layers.0.kernel\_i... &                                      glorot\_normal \\
                         feature\_rnn.n\_states &                                                 64 \\
                         feature\_rnn.n\_layers &                                                  1 \\
                    feature\_rnn.bidirectional &                                               True \\
                        feature\_rnn.cell\_type &                                                gru \\
        feature\_rnn.initial\_mlp.prefix\_length &                                                  1 \\
  feature\_rnn.initial\_mlp.layers.0.... &                          Choice([16, 32, 64, 128]) \\
  feature\_rnn.initial\_mlp.layers.0.... &   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
  feature\_rnn.initial\_mlp.layers.1.... &                          Choice([16, 32, 64, 128]) \\
  feature\_rnn.initial\_mlp.layers.1.... &   Choice(['softsign', 'softplus', 'relu', 'tanh']) \\
                          emission.scale\_kind &                                              fixed \\
                               emission.scale &  Choice([0.1, 0.2689655172413793, 0.43793103448... \\
               emission.layers.0.units &                                                 64 \\
          emission.layers.0.activation &                                           softplus \\
  emission.layers.0.kernel\_initializer &                                      glorot\_normal \\
                                     n\_hidden &                                                 64 \\
\bottomrule
\end{tabular}



==> tex/abstract.tex <==
Amortised inference enables scalable learning of sequential latent-variable models (LVMs) with the evidence lower bound (ELBO).
In this setting, variational posteriors are often only partially conditioned.
While the true posteriors depend, \eg, on the entire sequence of observations, approximate posteriors are only informed by past observations.
This mimics the Bayesian filter---a mixture of smoothing posteriors. 
Yet, we show that the ELBO objective forces partially-conditioned amortised posteriors to approximate products of smoothing posteriors instead.
Consequently, the learned generative model is compromised.
We demonstrate these theoretical findings in three scenarios: traffic flow, handwritten digits, and aerial vehicle dynamics.
Using fully-conditioned approximate posteriors, performance improves in terms of generative modelling and multi-step prediction.


==> tex/conclusion.tex <==
\section{Discussion \& Conclusion}
We studied the effect of leaving out conditions of amortised posteriors, presenting strong theoretical findings and empirical evidence that it can impair maximum likelihood solutions and inference.
Our work helps with approximate posterior design and provides intuitions for when full conditioning is necessary.
We advocate that partially-conditioned approximate inference models should be used with caution in downstream tasks as they may not be adequate for the task, \eg, replacing a Bayesian filter.
In general, we recommend conditioning inference models conforming to the true posterior.


==> tex/introduction.tex <==
\section{Introduction}
Variational inference has paved the way towards learning deep latent-variable models (LVMs): maximising the evidence lower bound (ELBO) approximates maximum likelihood learning \citep{jordan_introduction_1999,beal_variational_2003,mackay_information_2003}.
An efficient variant is amortised variational inference where the approximate posteriors are represented by a deep neural network, the inference network \citep{hinton_wake-sleep_1995}.
It produces the parameters of the variational distribution for each observation by a single forward pass---in contrast to classical variational inference  with a full optimisation process per sample.
The framework of variational auto-encoders \citep{kingma_auto-encoding_2014,rezende_stochastic_2014} adds the reparameterisation trick for low-variance gradient estimates of the inference network.
Learning of deep generative models is hence both tractable and flexible, as all its parts can be represented by neural networks and fit by stochastic gradient descent.

The quality of the solution is largely determined by how well the true posterior is approximated:
the gap between the ELBO and the log marginal likelihood is the KL divergence from the approximate to the true posterior.
Recent works have proposed ways of closing this gap, suggesting tighter alternatives to the ELBO \citep{burda_importance_2016,mnih_variational_2016} or more expressive variational posteriors \citep{rezende_variational_2015,mescheder_adversarial_2017}.
\citet{cremer_inference_2018} provide an analysis of this gap, splitting it in two.
The \emph{approximation gap} is caused by restricting the approximate posterior to a specific parametric form, the variational family.
The \emph{amortisation gap} comes from the inference network failing to produce the optimal parameters within the family.

In this work, we address a previously unstudied aspect of amortised posterior approximations: successful approximate posterior design is not merely about picking a parametric form of a probability density.
It is also about carefully deciding which conditions to feed into the inference network.
This is a particular problem in sequential LVMs, where it is common practice to feed only a restricted set of inputs into the inference network:
not conditioning on latent variables from other time steps can vastly improve efficiency \citep{bayer_learning_2014,lai_re-examination_2019}.
Further, leaving out observations from the future structurally mimics the Bayesian filter, useful for state estimation in the control of partially observable systems \citep{karl_unsupervised_2017,hafner_learning_2019,lee_stochastic_2020}.

We analyse the emerging \emph{conditioning gap} and the resulting suboptimality for sequential amortised inference models.
If the variational posterior is only partially conditioned, all those posteriors equal \wrt included conditions but different on the excluded ones will need to share an approximate posterior. 
The result is a suboptimal compromise over many different true posteriors which cannot be mitigated by improving variational family or inference network capacity. 
We empirically show its effects in an extensive study on three real-world data sets on the common use case of variational state-space models.

\begin{figure}[t]
	\includegraphics[width=\linewidth]{figures/bimodal.pdf}
	\caption{
        Illustration of the effect of partial conditioning.
        Consider a latent-variable model $\p{\incond, \outcond}{\latent} \times \p{\latent}$, with binary $\outcond$ and arbitrary $\incond$.
        We omit $\outcond$ from the \emph{amortised} approximate posterior $\q{\blatent}{\incond}$. 
        Shown are two cases of separated (left) and overlapping (right) Gaussian true posteriors.
        \textbf{Top row}: the full posteriors $\color{denimblue}\p{\latent}{\incond, \outcond=0}$ and $\color{palered}\p{\latent}{\incond, \outcond=1}$ as well as their average, the marginal posterior $\color{dark}\p{\latent}{\incond}$.
        \textbf{Middle row}: Variational Gaussian approximation $\color{dustyorange}\v{\blatent}{\incond}$ to the marginal posterior, which was obtained by stochastic gradient descent on the reverse, mode-seeking KL-divergence \citep{hoffman_stochastic_2013}.
        \textbf{Bottom row}: The optimal $\color{petrol}\w{\latent}{\incond}$ obtained by optimising the ELBO with a partially-conditioned amortised approximate posterior \wrt $\q$.
        It is located far away from the modes, sharply peaked and shares little mass with the true full posteriors, the marginal posterior as well as the approximate marginal posterior.
	}
	\label{fig:bimodal}
\end{figure}


==> tex/partial_conditioning.tex <==
\section{Partial Conditioning of Inference Networks}
\label{sec:partial_conditioning}
\begin{table}
	\caption{
		Overview of partial conditions for sequential inference networks $\q{\blatent_t}{\incond_t}$ in the literature.
		$\outcond_t$ denotes missing conditions vs.\  the true posterior according to the respective graphical model.
		DKF acknowledges the true factorization, but does not use $\blatent_{t-1}$ in any experiments.
%		All except STORN and VRNN learn a state-space model, their posteriors are thus independent of $\blatent\tsm{2}$.
%		DVBF additionally has $\bobs\Ts \in \incond_1$.
	}
	\label{tab:overview}
	\vskip.5em
	\centering
	\small
	\begin{tabular}{lll}
		\toprule
		Model & $\incond_t$ & $\outcond_t$ \\
		\midrule
		STORN  \citep{bayer_learning_2014} & $\bobs\Ts$ & $\blatent\tsm$  \\
        VRNN \citep{chung_recurrent_2015}  & $\bobs\ts, \blatent\tsm$ & $\bobs_{t+1:T}$  \\
		DKF \citep{krishnan_deep_2015}  &$\bobs\Ts$ & $\blatent\tm$ (exper.) \\
		DKS \citep{krishnan_structured_2017} & $\blatent\tm,\bobs_{t:T}$ & --\\
		DVBF \citep{karl_deep_2017}  & $\bobs_{t}, \blatent_{t-1}$ & $\bobs_{t+1:T}$  \\
		%SRNN \citep{fraccaro_sequential_2016} & $\bobs\Ts, \blatent\tm$ & --  \\
		Planet \citep{hafner_learning_2019}  & $\bobs_{t}, \blatent_{t-1}$& $\bobs_{t+1:T}$ \\
		SLAC \citep{lee_stochastic_2020}  & $\bobs_{t}, \blatent_{t-1}$& $\bobs_{t+1:T}$ \\
		\bottomrule
	\end{tabular}
\end{table}
VAEs add an additional consideration to approximate posterior design compared to classical variational inference: the choice of inputs to the inference networks.
Instead of feeding the entire observation $\bobs$, one can choose to feed a strict subset $\incond \subset \bobs$.
This is common practice in many sequential variants of the VAE, cf.\ \cref{tab:overview}, typically motivated by efficiency or downstream applications.
The discrepancy between inference models inputs and the true posterior conditions has been acknowledged before, \eg by \citet{krishnan_structured_2017}, where they investigate different variants.
Their analysis does not go beyond quantitative empirical comparisons.
In the following, we show that such design choices lead to a distinct third cause of inference suboptimality, the \emph{conditioning gap}.

\subsection{Minimising Expected KL Divergences Yields Products of Posteriors}
\label{sec:average_kl}
The root cause is that all observations $\bobs$ that share the same included conditions $\incond$ but differ in the excluded conditions must now share the same approximate posterior by design.
This shared approximate posterior optimizes the \emph{expected} KL divergence
\eq{
	\w := \arg\min_{\q} \expc[\outcond\mid\incond]{\kl{\q[\infpars]{\blatent|\incond}}{\p{\blatent | \incond,\outcond}}}.\label{eq:shared_posterior}\numberthis
}
\wrt the missing conditions $\outcond = \bobs \setminus \incond$.
By rearranging (cf. \cref{appendix:average_kl} for details)
\eq{
	&\expc[\outcond\mid\incond]{\kl{\q[\infpars]{\blatent|\incond}}{\p{\blatent | \incond,\outcond}}}\\
	= &
	\kl{
		\q[\infpars]{\blatent|\incond}
	}
	{
		\exp \mleft ( 	\expc[\outcond\mid\incond]{\log \p{\blatent | \incond,\outcond}} \mright) / \partition
	}
	- \log \partition,
}
where $\partition$ denotes a normalising constant, we see that the shared optimal approximate posterior is
\begin{align*}
	\w{\blatent} \propto \exp \mleft ( \expc[\outcond\mid\incond]{\log \p{\blatent | \incond,\outcond}} \mright).
\end{align*}
Interestingly, this expression bears superficial similarity with the true partially-conditioned posterior
\begin{align*}
	\p{\blatent}{\incond} = \expc[\outcond\mid\incond]{\p{\blatent|\incond,\outcond}} = \exp\mleft(\log\mleft(\expc[\outcond\mid\incond]{\p{\blatent|\incond,\outcond}}\mright)\mright).
\end{align*}
To understand the difference, consider a uniform discrete $\outcond\mid\incond$ for the sake of the argument.
In this case, the expectation is an average over all missing conditions.
The true posterior $\p{\blatent|\incond}$ is then a mixture distribution of all plausible full posteriors $\p{\blatent|\incond,\outcond}$.
The optimal approximate posterior, because of the logarithm inside the sum, is a \emph{product} of plausible full posteriors. 
Such distributions occur \eg in products of experts \citep{hinton_training_2002} or Gaussian sensor fusion \citep{murphy_machine_2012}.
Products behave differently from mixtures:
%an intuition provided by \citet{Welling2007} is that products aim for a consensus, since each factor can single-handedly ``veto'' a sample, while each term in a mixture can only ``pass'' it.
an intuition due to \citet{welling_product_2007} is that a factor in a product can single-handedly ``veto'' a sample, while each term in a mixture can only ``pass'' it.

This intuition is highlighted in \cref{fig:bimodal}.
We can see that $\w$ is located between the modes and sharply peaked.
It shares almost no mass with both the posteriors and the marginal posterior.
The approximate marginal posterior $\v$ on the other hand either covers one or two modes, depending on the width of the two full posteriors–-a much more reasonable approximation.

In fact, $\w{\blatent}$ will only coincide with either $\p{\blatent}{\incond}$ or $\p{\blatent}{\incond, \outcond}$ in the the extreme case when $\p{\blatent}{\incond} = \p{\blatent}{\incond, \outcond} \Leftrightarrow \p{\blatent}{\incond} \p{\outcond}{\incond} = \p{\blatent, \outcond}{\incond}$, \cf \cref{app:conditioning_optimum}, which implies statistical independence of $\outcond$ and $\blatent$ given $\incond$.

Notice how the suboptimality of $\w$ assumed neither a particular variational family, nor imperfect amortisation---$\w$ is the analytically optimal shared posterior.
Both approximation and amortisation gap would only additionally affect the KL divergence inside the expectation in \cref{eq:shared_posterior}.
As such, the inference suboptimality described here can occur even if those vanish.
We call 
\begin{equation}
	\expc[\incond]{\expc[\outcond\mid\incond]{\kl{\w{\blatent | \incond}}{\p{\blatent | \incond,\outcond}}}}
\end{equation}
the \emph{conditioning gap}, which in contrast to approximation and amortisation gap can only be defined as an expectation \wrt $\p{\bobs} = \p{\outcond, \incond}$.

Notice further that the effects described here assumed the KL divergence, a natural choice due to its duality with the ELBO (cf.\ \cref{eq:elbo}).
To what extent alternative divergences \citep{ranganath_black_2014,li_renyi_2016} exhibit similar or more favourable behaviour is left to future research.

\paragraph{Learning Generative Models with Partially-Conditioned Posteriors}
We find that the optimal partially-conditioned posterior will not correspond to desirable posteriors such as ${\p{\blatent}{\incond}}$ or ${\p*{\blatent}{\incond, \outcond}}$, even assuming that the variational family could represent them.
This also affects learning the generative model.
A simple variational calculus argument (\cref{app:proof_generative}) reveals that, when trained with partially-conditioned approximate posteriors, maximum-likelihood models and ELBO-optimal models are generally not the same.
In fact, they coincide only in the restricted cases where $\p*{\blatent}{\incond, \outcond}=\q{\blatent}{\incond}$.
As seen before this is the case if and only if $\outcond \perp \blatent\mid\incond$.


\subsection{Learning a Univariate Gaussian}
\label{sec:example}
It is worth highlighting the results of this section in a minimal scalar linear Gaussian example.
The target distribution is $\target{x} \sim \gauss{0, 1}$.
We assume the latent variable model
\begin{equation*}
	\p[a]{\obs,\latent} = \gauss{\obs|a\latent, 0.1}\cdot\gauss{\latent|0, 1}
\end{equation*} 
with free parameter $a\geq0$.
This implies
\eq{
	\p[a]{\obs} = \gauss{\obs|
		0, 0.1 + a^2},\quad
	\p[a]{\latent}{\obs} = \gauss{\latent|a\mleft(0.1+a^2\mright)^{-1}x, \mleft(1+10a^2\mright)^{-1}}.
}
With $a^*=\sqrt{0.9}$, we recover the target distribution with posterior
$\p[a^*]{\latent}{\obs} = \gauss{\latent|\sqrt{0.9}\obs, 0.1}$.
Next, we introduce the variational approximation
$\q{\latent} = \gauss*{\latent|\mu_\latent, \sigma_\latent^2 }$.
With the only condition $\obs$ missing, this is a deliberately extreme case of partial conditioning where $\incond=\emptyset$ and $\outcond=\{x\}$.
Notice that the true posterior is  a member of the variational family, \ie, no approximation gap.
We maximise the \emph{expected} ELBO
\eq{
	\w[a]{\latent} = \arg\max_q \expc[\obs\sim\emp]{\expc[\latent \sim q]{\log \frac{\p[a]{\obs, \latent}}{\q{\latent}}}},
}
\ie, all observations from $\hat{p}$ share the same approximation $\q$.
One can show that
\begin{equation*}
\w[a]{\latent} = 	\gauss{\latent|0, \mleft(100a^2 + 1\mright)^{-1} }.
\end{equation*}
We immediately see that $\w[a]{\latent}$ is neither equal to $\p[a^*]{\latent}{\obs} \equiv \p{\latent}{\incond,\outcond}$ nor to $\p{\latent}\equiv\p{\latent}{\incond}$.
Less obvious is that the variance of the optimal solution is much smaller than that of both $\p{\latent}{\incond,\outcond}$ and $\p{\latent}{\incond}$.
This is a consequence of the product of the \emph{expert compromise} discussed earlier: the (renormalised) product of Gaussian densities will always have lower variance than either of the factors.
This simple example highlights how poor shared posterior approximations can become.

Further, inserting $\w[a]$ back into the expected ELBO and optimising for $a$ reveals that the maximum likelihood model parameter $a^*$ is not optimal.
In other words, $\p[a^*]{\obs, \latent}$ does not optimise the expected ELBO in $p$---despite being the maximum likelihood model.


\subsection{Extension to the Sequential Case}
\label{sec:sequential_case}
The conditioning gap may arise in each of the terms of \cref{eq:sequential_kl} if $q$ is partially conditioned.
Yet, it is common to leave out future observations, \eg $\q{\blatent_t}{\blatent\tsm, \bobs\ts, \cancel{\bobs_{t+1:T}}}$.
To the best of our knowledge, in the literature only sequential applications of VAEs are potentially affected by the conditioning gap.
Still, sequential latent-variable models with amortised under-conditioned posteriors have been applied success fully to, \eg, density estimation, anomaly detection, and sequential decision making \citep{bayer_learning_2014,soelch_variational_2016,hafner_learning_2019}.
This may seem at odds with the previous results.
The gap is not severe in all cases.
%It is problematic when the discrepancy between the true posteriors, \cref{eq:filterbias},
%is not constant in $\blatent_t$.
%This is a property of \emph{both the model and the empirical distribution}, over which the expectation is taken.
Let us emphasize two ``safe'' cases where the gap vanishes because  $\outcond_t \perp \blatent_t~|~\incond_t$ is approximately true.
First, where the partially- and the fully-conditioned posterior correspond to the prior transition, \ie 
\begin{equation*}
	\p{\blatent_t}{\blatent_{t-1}} \approx \p{\blatent_t}{\incond_t}\approx \p{\blatent_t}{\incond_t, \outcond_t}.
\end{equation*}
This is for example the case for deterministic dynamics where the transition is a single point mass.
Second, the case where the observations are sufficient to explain the latent state, \ie 
\begin{equation*}
	\p{\blatent_t}{\bobs_t} \approx \p{\blatent_t}{\incond_t}\approx \p{\blatent_t}{\incond_t, \outcond_t}.
\end{equation*}
A common case are systems with perfect state information.

Several studies have shown that performance gains of fully-conditioned over partially-conditioned approaches are negligible \citep{fraccaro_sequential_2016,maddison_filtering_2017,buesing_learning_2018}.
We conjecture that the mentioned ``safe'' cases are overrepresented in the studied data sets.
For example, environments for reinforcement learning such as the gym or MuJoCo environments \citep{todorov_mujoco_2012,brockman_openai_2016} feature deterministic dynamics.  
We will address a broader variety of cases in \cref{sec:statespacestudy}.



==> tex/preliminaries.tex <==
\section{Amortised Variational Inference}
\subsection{Variational Auto-Encoders}
Consider the task of fitting the parameters of a latent-variable model 
$\p[\genpars]{\bobs, \blatent} = \p[\genpars]{\bobs}{\blatent} \times \p[\genpars]{\blatent}$ 
to a target distribution $\target{\bobs}$ by maximum likelihood:
\eq{
	\arg\max_{\genpars}~\expc[\bobs \sim \target{\bobs}]{\log \p[\genpars]{\bobs}}. \numberthis \label{eq:ml}
}
In the case of variational auto-encoders (VAEs), the prior distribution $\p[\genpars]{\blatent}$ is often simple, such as a standard Gaussian. 
The likelihood $\p[\genpars]{\bobs}{\blatent}$ on the other hand is mostly represented by a deep neural network producing the likelihood parameters as a function of $\blatent$.

The log marginal likelihood $\log \p[\genpars]{\bobs} = \log \int \p[\genpars]{\bobs, \blatent}
\dint \blatent$ contains a challenging integral within a logarithm.
The maximisation of \cref{eq:ml} is thus generally intractable.
Yet, for a single sample $\bobs$ the log marginal likelihood can be bounded from below by the evidence lower bound (ELBO):
\eq{
	\log \p[\genpars]{\bobs} &\ge  \log \p[\genpars]{\bobs} - \kl{\q{\blatent}}{\p[\genpars]{\blatent}{\bobs}} \numberthis \label{eq:elbo} \\
	&= \expc[\blatent \sim q]{\log \p[\genpars]{\bobs}{\blatent}} - \kl{\q{\blatent}}{\p[\genpars]{\blatent}} =: -\ell(\genpars, q, \bobs),
}
where a surrogate distribution $\q$, the variational posterior, is introduced. 
The bound is tighter the better $\q{\blatent}$ approximates $\p[\genpars]{\blatent}{\bobs}$.
The gap vanishes with the posterior KL divergence in \cref{eq:elbo}. 

Typically, the target distribution is given by a finite data set $\dataset = \{\bobs^{(n)}\}_{n=1}^N$. 
In classical variational inference, equally many variational posteriors $\{q^{(n)}(\blatent) \}_{n=1}^N$ are determined by direct optimisation. 
For instance, each Gaussian $q^{(n)}(\blatent)$ is represented by its mean $\mu^{(n)}$ and standard deviation $\sigma^{(n)}$. The set of all possible distributions of that parametric form is called the variational family $ \varfam \ni \q{\blatent}$.
Learning the generative model parameters $\genpars$ can then be performed by an empirical risk minimisation approach, where the average negative ELBO over a data set is minimised:
\eq{
	\arg\min_{\genpars, \{q^{(n)}\}_{n=1}^N}~\sum_{n=1}^N  \ell\mleft(\genpars, q^{(n)}(\blatent), \bobs^{(n)}\mright).
}
The situation is different for VAEs.
The parameters of the approximate posterior for a specific sample~$\bobs$ are produced by another deep neural network, the inference network $\q[\infpars]{\blatent}{\bobs}$. Instead of directly optimising for sample-wise parameters, a global set of weights $\phi$ for the inference network is found by stochastic gradient-descent of the expected negative ELBO:
\eq{
	\arg\min_{\genpars, \infpars}~\expc[\bobs \sim \target{\bobs}]{\ell \mleft (\genpars, \q[\infpars]{\blatent}{\bobs}, \bobs \mright )}.
}
This approach tends to scale more gracefully to large data sets.

\paragraph{The Sequential Case} 
The posterior of a sequential latent-variable model 
\begin{equation*}
	\p{\bobs\Ts, \blatent\Ts} = \prod_{t=1}^T \p{\bobs_t}{\bobs\tsm,\blatent\ts} \p{\blatent_t}{\blatent\tsm, \bobs\tsm}.
\end{equation*}
of observations 
$(\bobs_1, \dots, \bobs_T) = \bobs\Ts$ 
and latents 
$(\blatent_1, \dots, \blatent_T) = \blatent_{1:T}$, with $\blatent_{1:0} = \emptyset$, factorises as
\eq{
	\p{\blatent\Ts}{\bobs\Ts} = \prod_{t=1}^T \p{\blatent_t}{\blatent\tsm, \bobs\Ts}. \numberthis \label{eq:true_posterior}
}
The posterior KL divergence is a sum of step-wise divergences \citep{cover_elements_2006}:
\eq{
	\kl*{\q{\blatent\Ts}{\cdot}}{\p{\blatent\Ts}{\bobs\Ts}} =
	\sum_{t=1}^T \expc*[\blatent_{1:t-1} \sim q]{
		\kl{
			\q{\blatent_t}{\cdot}
		}{
			\p{\blatent_t}{\blatent\tsm, \bobs\Ts}
		}
    }\numberthis \label{eq:sequential_kl}
}
where we have left out the conditions of $\q{\blatent\Ts}{\cdot} = \prod_t \q{\blatent_t}{\cdot}$ for now.
This decomposition allows us to focus on the non-sequential case in our theoretical analysis, even though the phenomenon most commonly occurs with sequential LVMs.
%In particular, each factor depends on multiple conditions, only some of which are typically dropped in approximate posteriors.
%We denote the set of included conditions at each time step by $C_t$, while the left out ones are collected in $\outcond_t$, \ie $\incond_t\,\dot\cup\,\outcond_t = \{\blatent_{1:\tminus1},\bobs\Ts\}$. 
%With this notation, the true posterior and the partially-conditioned amortised posterior are
%\vspace{-.35em}
%\eq{
%	\p{\blatent\Ts}{\bobs\Ts} &= \prod_{t=1}^T \p{\blatent_t}{\incond_t, \outcond_t}, \numberthis\label{eq:cond_true_posterior}\\[-.1em]
%	\q{\blatent\Ts}{\bobs\Ts} &= \prod_{t=1}^T \q{\blatent_t}{\incond_t}, \numberthis\label{eq:cond_apx_posterior}
%}
%respectively. 
%Partial conditions are common practice in the recent literature, see \cref{tab:overview} for examples.


\subsection{The Approximation and Amortisation Gaps}
The ELBO and the log marginal likelihood are separated by the posterior Kullback-Leibler divergence $\kl{\q{\blatent}}{\p[\genpars]{\blatent}{\bobs}}$, cf.\ \cref{eq:elbo}. 
If the optimal member of the variational family $q^\star \in \varfam$ is not equal to the true posterior, or $\p{\blatent}{\bobs} \notin \varfam$, then
\eq{
	\kl{\optq{\blatent}}{\p[\genpars]{\blatent}{\bobs}} > 0,
}
so that the ELBO is strictly lower than the log marginal likelihood---the \emph{approximation gap}.

Using an inference network we must expect that even the optimal variational posterior within the variational family is not found in general.
The gap widens:
\eq{
	\kl{\q[\infpars]{\blatent}{\bobs}}{\p[\genpars]{\blatent}{\bobs}} \ge \kl{\optq{\blatent}}{\p[\genpars]{\blatent}{\bobs}}.
}
This phenomenon was first discussed by \citet{cremer_inference_2018}.
The additional gap 
\eq{
	\kl{\q[\infpars]{\blatent}{\bobs}}{\p[\genpars]{\blatent}{\bobs}} - \kl{\optq{\blatent}}{\p[\genpars]{\blatent}{\bobs}} \ge 0.
}
is called the \emph{amortisation gap}.

The two gaps represent two distinct suboptimality cases when training VAEs. 
The former is caused by the choice of variational family, the latter by the success of the amortised search for a good candidate $q \in \varfam$.


==> tex/relatedwork.tex <==
\section{Related Work}
\label{sec:related_work}
The bias of the ELBO has been studied numerous times \citep{nowozin_debiasing_2018,huang_note_2019}.
A remarkable study by \citet{cemgil_two_2011} contains a series of carefully designed experiments showing how different forms of assumptions on the approximate posterior let different qualities of the solutions emerge.
This study predates the introduction of amortised inference \citep{kingma_auto-encoding_2014,rezende_stochastic_2014} however.
\citet{cremer_inference_2018} identify two gaps arising in the context of VAEs:
the approximation gap, \ie inference error resulting from the true posterior not being a member of variational family;
and the amortisation gap, \ie imperfect inference due to an amortised inference procedure, \eg a single neural network call.
Both gaps occur \emph{per sample} and are independent of the problems  in \cref{sec:partial_conditioning}.

Applying stochastic gradient variational Bayes \citep{kingma_auto-encoding_2014,rezende_stochastic_2014} to sequential models was pioneered by \citet{bayer_learning_2014,fabius_variational_2015,chung_recurrent_2015}.
The inclusion of state-space assumptions was henceforth demonstrated by \citet{archer_black_2015,krishnan_deep_2015,krishnan_structured_2017,karl_deep_2017,fraccaro_sequential_2016,fraccaro_disentangled_2017,becker-ehmck_switching_2019}.
Specific applications to various domains followed, such as video prediction \citep{denton_stochastic_2018}, tracking \citep{kosiorek_sequential_2018,hsieh_learning_2018,akhundov_variational_2019} or simultaneous localisation and mapping \citep{mirchev_approximate_2019}.
Notable performance in model-based sequential decision making has also been achieved by \citet{gregor_temporal_2019,hafner_learning_2019,lee_stochastic_2020,karl_unsupervised_2017,becker-ehmck_learning_2020}.
The overall benefit of latent sequential variables was however questioned by \citet{lai_re-examination_2019}.
The performance of sequential latent-variable models in comparison to auto-regressive models was studied, arriving at the conclusion that the added stochasticity does not increase, but even decreases performance. 
We want to point out that their empirical study is restricted to the setting where $\blatent_t \perp \blatent\tsm ~|~ \bobs\Ts$, see the appendix of their work.
We conjecture that such assumptions lead to a collapse of the model where the latent variables merely help to explain the data local in time, \ie intra-step correlations.

A related field is that of \emph{missing-value imputation}.
Here, tasks have increasingly been solved with probabilistic models \citep{ledig_photo-realistic_2017,ivanov_variational_2019}.
The difference to our work is the explicit nature of the missing conditions.
Missing conditions are typically directly considered by learning $\p{\outcond|\incond}$ instead of $\p{\bobs}$ and appropriate changes to the loss functions.


==> tex/statespacestudy.tex <==
\section{Study: Variational State-Space Models}
\label{sec:statespacestudy}
We study the implications of \cref{sec:partial_conditioning} for the case of variational state-space models (VSSMs).
We deliberately avoid the cases of deterministic dynamics and systems with perfect state information: unmanned  aerial vehicle (UAV) trajectories with imperfect state information in \cref{sec:blackbird}, a sequential version of the MNIST data set \cref{sec:mnist} and traffic flow in \cref{sec:traffic_flow}.
The reason is that the gap is absent in these cases, see \cref{sec:sequential_case}.
%We tackle prediction of unmanned aerial vehicle (UAV) trajectories \citep{antonini2018blackbird} several time steps into the future in \cref{sec:blackbird}.
%By leaving out the rotational information from the observations we mimic a system with imperfect state information.
%We then revisit a classic data set, MNIST, which we cast as a sequential problem in \cref{sec:mnist} by considering rows of pixels from top to bottom. 
%This is a stochastic system---for instance, the digits 0, 3, 8 and 9 all start with a round line.
%It also has a higher dimensionality of 28, bearing potential for significant intra-step correlations.
%Finally we consider a data set of traffic flow in \cref{sec:traffic_flow}.
%Its most prominent feature is a high degree of stochasticity in its dynamics even though we treat only a single of its dimensions.
In all cases, we not only report the ELBO, but conduct qualitative evaluations as well.
We start out with describing the employed model in \cref{sec:vrssm_implementation}.

%Exploiting that state-of-the-art classifiers are easily available for that data set lets us test whether under- and fully-conditioned models are on par \wrt the class distribution that is induced by the respective learned models.

%For results comparing the conditioning of models that are auto-regressive in both latent and observed variables, we point the reader to \citep{MaddisonLTHNMDT17,Chung2015recurrent}.

\subsection{Variational State-Space Models}
\label{sec:vrssm_implementation}
The two Markov assumptions that every observation only depends on the current state and every state only depends on the previous state and condition lead to the following generative model:
%\vspace{-.75em}
\begin{equation*}
    \p{\bobs\Ts, \blatent\Ts}{\bcond\Ts} = \prod_{t=1}^T \p{\bobs_t}{\blatent_t} \p{\blatent_t}{\blatent_{t-1}, \bcond_{t-1}},
\end{equation*}
where $\bcond\Ts$ are additional conditions from the data set (such as control signals) and $\blatent_{0} = \bcond_{0} := \emptyset$.
We consider three different conditionings of the inference model
%\vspace{-.5em}
\begin{equation*}
    \q{\blatent\Ts}{\bobs\Ts,\bcond\Ts} = \q{\blatent_1}{\bobs_{1:k},\bcond_{1:k}} \prod_{t=2}^T \q{\blatent_t}{\blatent_{t-1}, \bobs_{1:m},\bcond_{1:m}},
\end{equation*}
\emph{partial} with $k=1, m=t$, \emph{semi} with $k > 1, m=t$,  and \emph{full} with $k=m=T$.
We call $k$ the \emph{sneak peek}, inspired by \citet{karl_deep_2017}.
See \cref{sec:vrssm_implementation_details} for more details.

\subsection{UAV Trajectories from the Blackbird Data Set}
\label{sec:blackbird}
\begin{figure}
	\begin{subfigure}[t]{.49\linewidth}
		\includegraphics[width=\linewidth]{figures/blackbird/ppc-semi-full-test-0}
		\caption{x-axis}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{.49\linewidth}
		\includegraphics[width=\linewidth]{figures/blackbird/ppc-semi-full-test-1}
		\caption{y-axis}
	\end{subfigure}
	\caption{
		Posterior-predictive check of prefix-sampling on the Blackbird data set.
		Possible futures 
		%$\hat \bobs_{t+1:T}^{(i)}$ 
		are sampled from the model after having observed a prefix $\bobs_{1:t}$.
		The state at the end of the prefix is inferred with a bootstrap particle filter.
		Each plot shows a kernel density estimate of the distribution over the final location $\bobs_T$, once for the semi-conditioned model in \textcolor{semi}{green} and for the fully-conditioned in \textcolor{full}{blue}.
		The true value is marked as a vertical, black line.
		The fully-conditioned model assigns higher likelihood in almost all cases and is more concentrated around the truth.
	}
	\label{fig:blackbird-ppc}
\end{figure}

We apply semi- and fully-conditioned VSSMs to UAV modelling \citep{antonini_blackbird_2018}.
By discarding the rotational information, we create a system with imperfect state information, \cf \cref{sec:sequential_case}.
Each observation $\bobs_t \in \RR^3$ is the location of an unmanned aerial vehicle (UAV) in a fixed global frame.
The conditions $\bcond_t \in \RR^{14}$, consist of IMU readings, rotor speeds, and pulse-width modulation.
The emission model was implemented as a Gaussian with fixed, hand-picked standard deviations, where the mean corresponds to the first three state dimensions (cf. \citep{akhundov_variational_2019}):
$\p{\bobs_t}{\blatent_t} = \mathcal{N}\mleft(\boldsymbol{\mu}=\blatent_{t, 1:3}, \boldsymbol{\sigma}^2=[0.15, 0.15, 0.075]\mright)$.
We leave out the partially-conditioned case, as it cannot infer the higher-order derivatives necessary for rigid-body dynamics.
A \emph{sneak peek} of $k=7$ for the semi-conditioned model is theoretically sufficient to infer those moments.
See \cref{sec:blackbird_details} for details.

Fully-conditioned models outperform semi-conditioned ones on the test set ELBO, as can be seen in \cref{tab:blackbird-traffic-elbo}.
We evaluated the models on prefix-sampling, \ie the predictive performance of $\p{\bobs_{t+1:T}}{\bobs_{1:t}, \bcond_{1:T}}$.
To restrict the analysis to the found parameters of the generative model only, we inferred the filter distribution $\p{\blatent_t}{\bobs\ts, \bcond\ts}$ using a bootstrap particle filter \citep{sarkka_bayesian_2013}.
By not using the respective approximate posteriors, we ensure fairness between the different models.
Samples from the predictive distribution were obtained via ancestral sampling of the generative model.
Representative samples are shown in \cref{fig:rollout-prefix-sampling}.
We performed a posterior-predictive check for both models, where we compare the densities of the final observations $\bobs_T$ obtained from prefix sampling in \cref{fig:blackbird-ppc}.
Both evaluations qualitatively illustrate that the predictions of the fully-conditioned approach concentrate more around the true values. In particular the partially-conditioned model struggles more with long-term prediction.

\begin{table}[t]
    \caption{Results on UAV and row-wise MNIST modelling.}
    \begin{subtable}[t]{.475\linewidth}
    	\caption{
    		ELBO values for models with differently conditioned variational posteriors for various data sets. 
    		Presented values are averages over ten samples from the inference model. 
    		The standard deviations were negligible.
    		Higher is better.
    	}
    	\hspace{0.2cm}
    	\label{tab:blackbird-traffic-elbo}
    	\centering
    	\small
    	\begin{tabular}{lll|ll}
    		\toprule
    		& \multicolumn{2}{c}{UAV} & \multicolumn{2}{c}{Traffic Flow} \\
    		& val    & test  & val   & test       \\
    		\multicolumn{1}{l}{partial} & -      & -     & $-2.91$ & $-2.97$\\
    		\multicolumn{1}{l}{semi}    & $1.47$ & $2.13$& $-2.73$ & $-2.75$\\
    		\multicolumn{1}{l}{full}    & $2.03$ & $2.41$& $-2.69$ & $-2.78$\\
    		\bottomrule
    	\end{tabular}
    	
    	% With train errors.
    	%\begin{tabular}{llll|lll}
    	%\toprule
    	%                            & \multicolumn{3}{c}{UAV} & \multicolumn{3}{c}{Traffic Flow} \\
    	%                            & train  & val    & test  & train & val   & test       \\
    	%\multicolumn{1}{l}{partial} & -      & -      & -     & $-2.81$ & $-2.91$ & $-2.97$\\
    	%\multicolumn{1}{l}{semi}    & $2.29$ & $1.47$ & $2.13$& $-2.46$ & $-2.73$ & $-2.75$\\
    	%\multicolumn{1}{l}{full}    & $2.82$ & $2.03$ & $2.41$& $-2.34$ & $-2.69$ & $-2.78$\\
    	%\bottomrule
    	%\end{tabular}
    \end{subtable}
    \hspace{.05\linewidth}
    \begin{subtable}[t]{.475\linewidth}
        \caption{
            Results for row-wise MNIST.
            We report the ELBO as a lower bound on the log-likelihood and the KL-Divergence of the digit distribution induced by the model from a uniform distribution.
            Other results by \citet{klushyn_learning_2019}.
        }
        %\vskip 0.1in
        \label{tab:mnist}
        \label{tab:mnist-ll}
        \centering
        \small
        \begin{tabular}{llll|lll}
            \toprule
            Distribution & Log-Likelihood $\uparrow$ & KL $\downarrow$ \\
            \midrule
            data & - & $0.002$ \\
            %partial & $\geq -98.9857 \pm 0.0565$  & $0.0980$ \\
            partial & $\geq -98.99 \pm 0.06$  & $0.098$ \\
            full  & $\geq -88.45 \pm 0.05$ &$0.015$\\
            \midrule
            vhp + rewo & $\geq -82.74$ & - \\
            iwae (L=2) & $\geq -82.83$ & - \\ 
            %vhp + geco & $\geq -96.32$ \\
            %VampPrior & $\geq -84.02$ \\
            %iwae (L=1) & $\geq -84.46$ \\ 
            \bottomrule
        \end{tabular}
    \end{subtable}
\end{table}

\begin{figure}[t]
	\centering
	\begin{subfigure}[t]{.45\linewidth}
		\begin{center}
			\includegraphics[width=\linewidth]{figures/rowing-mnist/mnist-hist.pdf}
		\end{center}
	\end{subfigure}
	\begin{subfigure}[t]{.54\linewidth}
		\begin{center}
			\includegraphics[width=\linewidth]{figures/rowing-mnist/mnist-samples.pdf}
		\end{center}
	\end{subfigure}
	\caption{
		\textbf{Left:}
		Class distributions of the respective image distributions induced by a state-of-the-art classifier.
		The data distribution is close to uniform, except for $5$.
		The fully-conditioned model yields too few $5$'s and is close to uniform for the other digits.
		The partially-conditioned model only captures the right frequencies of $1$ and $3$.
		\textbf{Right:}
		Comparison of generative sampling on row-wise MNIST.
		Samples from the data distribution are shown on the left. 
		The middle and right show samples from models with an partially- and a fully-conditioned approximate posterior, respectively.
	}
	\label{fig:mnist-qualitative}
\end{figure}

\subsection{Row-Wise MNIST}
\label{sec:mnist}
We transformed the MNIST data set into a sequential data set by considering one row in the image plane per time step, from top to bottom.
This results in stochastic dynamics: similiar initial rows can result in a 3, 8, 9 or 0, future rows are very informative (\cf \cref{sec:sequential_case}). 
Before all experiments, each pixel was binarised by sampling from a Bernoulli with a rate in $[0, 1]$ proportional to the corresponding pixel intensity.

The setup was identical to that of \cref{sec:blackbird}, except that a Bernoulli likelihood parameterised by a feed-forward neural network was used:
$\p{\bobs_t}{\blatent_t} = \mathcal{B}\mleft(\fnn{\genpars_E}{\blatent_t} \mright)$.
No conditions $\bcond\Ts$ and a short sneak-peek ($k=1$) were used.
The fully-conditioned model outperforms the partially-conditioned by a large margin, placing it significantly closer to state-of-the-art performance, see \cref{tab:mnist}.
This is supported by samples from the model, see \cref{fig:mnist-qualitative}.
\Cf \cref{sec:mnist_details} for details.

For qualitative evaluation, we used a state-of-the-art classifier%
\footnote{\url{https://github.com/keras-team/keras/blob/2.4.0/examples/mnist_cnn.py}}
to categorise 10,000 samples from each of the models.
If the data distribution is learned well, we expect the classifier to behave similarly on both data and generative samples, \ie yield uniformly distributed class predictions. 
We report KL-divergences from the uniform distribution of the class prediction distributions in \cref{tab:mnist}.
A bar plot of the induced class distributions can be found in \cref{fig:mnist-qualitative}.
Only the fully-conditioned model is able to nearly capture a uniform distribution. 
%The problem with the digit `5` seems to be rooted in the classifier, as the classifications of the test data err for that digit as well.

%data: [0.09902916 0.11380051 0.10195884 0.1011     0.09766012 0.08787084 0.09543987 0.10228471 0.10044064 0.1004153 ]
% KL from uniform: 0.0018692373996600509
% experiments/from-polyaxon/vssm-rowing-mnist/groups/139/14150/33/33/val-final.h5: [0.10845336 0.12270451 0.09053644 0.10423501 0.0950452  0.05734539  0.09805628 0.1084441  0.11117422 0.10400081]
%  KL from uniform: 0.015234032645821571
%  experiments/from-polyaxon/vssm-rowing-mnist/groups/140/14151/56/56/val-final.h5: [0.08663252 0.09809444 0.06745608 0.09933151 0.07581688 0.05596943 0.03589791 0.13509265 0.17358042 0.1721208 ]
%   KL from uniform: 0.09803376346826553

\subsection{Traffic Flow}
\label{sec:traffic_flow}
We consider the Seattle loop data set \citep{cui_deep_2019,cui_traffic_2020} of average speed measurements of cars at 323 locations on motorways near Seattle, from which we selected a single one (42).
The dynamics of this system are highly stochastic, which is of special interest for our study, \cf \cref{sec:sequential_case}.
Even though all days start out very similar, traffic jams can emerge suddenly.
In this scenario the emission model was a feed-forward network conditioned on the whole latent state, \ie
$\p{\bobs_t}{\blatent_t} = \mathcal{N}\mleft(\fnn{\genpars_E}{\blatent_t}, \sigma_x^2 \mright)$.
We compare partially-, semi- ($k=7$) and fully-conditioned models.
See \cref{sec:traffic_flow_details} for details.
The results are shown in \cref{tab:blackbird-traffic-elbo}.
While the fully-conditioned posterior emerges as the best choice on the validation set, the semi-conditioned and the fully-conditioned one are on par on the test set. 
We suspect that the \emph{sneak peek} is sufficient to fully capture a sensible initial state approximation.
%We also evaluated a closer estimate of the marginal log-likelihood, the importance-weighted lower bound \citep{BurdaGS15} making use of 10 samples.
%The bounds are very close (up to the third decimal), indicating that the difference in performance is more to the marginal log-likelihood than to the divergence of the variational posterior from the true posterior.
%Hence, the inconsistency of under-conditioning manifests itself in worse models, and not in worse posterior approximations.

We performed a qualitative evaluation of this scenario as well in the form of prefix sampling.
Given the first $t=12$ observations, the task is to predict the remaining ones for the day, compare \cref{sec:blackbird}.
We show the results in \cref{fig:rollout-prefix-sampling}.
The fully-conditioned model clearly shows more concentrated yet multi-modal predictive distributions.
The partially-condition model concentrates too much, and the semi-conditioned one too little.
%We conjecture that the full conditioning enables the learning algorithm to detect stochastic patterns much easier.
\setlength{\tabcolsep}{2pt}
\begin{figure}[t]
\centering
\begin{tabular}{m{.075\linewidth}m{.45\linewidth}m{.45\linewidth}}

 & UAV & Traffic Flow \\
\midrule

partial &
\centering - &
\includegraphics[width=1\linewidth]{figures/seattle-loop/prefix-samples-under-test} \\

semi &
\includegraphics[width=1\linewidth]{figures/blackbird/prefix-samples-semi-test} &
\includegraphics[width=1\linewidth]{figures/seattle-loop/prefix-samples-semi-test} \\

full &
\includegraphics[width=1\linewidth]{figures/blackbird/prefix-samples-full-test} &
\includegraphics[width=1\linewidth]{figures/seattle-loop/prefix-samples-full-test}
\end{tabular}
\caption{
	Comparison of prefix-sampling.
	Possible futures $\hat \bobs_{k+1:T}^{(i)}$ (coloured lines) are sampled from the model after having observed a prefix $\bobs_{1:k}$ (solid black line) and then compared to the true suffix $\bobs_{k+1:T}$ (dashed line).
	The state at the end of the prefix is inferred with a bootstrap particle filter.
	\textbf{Left:} UAV data, top-down view.
	\textbf{Right:} Traffic flow data, time-series view.
}\label{fig:vssm-blackbird}\label{fig:rollout-prefix-sampling}
%\vskip -0.2in
\end{figure}

